A Compiler-Compiler for DSL Embedding

In this paper, we present a framework to generate compilers for embedded domain-specific languages (EDSLs). This framework provides facilities to automatically generate the boilerplate code required for building DSL compilers on top of extensible optimizing compilers. We evaluate the practicality of our framework by demonstrating several use-cases successfully built with it.

==> related.tex <==
\section{Related Work}
\label{sec:related}
Yacc~\cite{johnson1975yacc} is a compiler-compiler for generating parsers specified using a declarative language.
There are numerous systems for
defining new languages, referred as language workbenches~\cite{fowler2005language,erdweg2013state}, such as Stratego/Spoofax~\cite{spoofax}, SugarJ~\cite{Erdweg:2011:SLS:2048066.2048099}, KHEPERA~\cite{khepera}, and MPS~\cite{mps}.

Stratego/Spoofax~\cite{spoofax} uses strategy-based
term-rewrite systems for defining optimizations for
a programming language. Stratego uses an approach similar to quasi-quotation~\cite{stratego-qq}
to hide the expression terms from the user. For the same purpose, \systemname uses
annotations for specifying a subset of optimizations specified by the compiler expert. 
One can use quasi-quotes~\cite{scala-qq,Parreaux:2017:QSR:3136040.3136043} for implementing  optimizations in concrete syntax (rather than abstract syntax) similar to Stratego.

Truffle~\cite{truffle-dsl} provides a DSL for defining
self-optimizing AST interpreters, using the Graal~\cite{graal} optimizing compiler as the backend. 
This system mainly focuses on providing just-in-time compilation for dynamically typed languages such as JavaScript and R, by annotating AST nodes.
In contrast, \systemname uses annotation on the library itself, and generates the AST nodes based on strategy defined by the compiler expert.

Forge~\cite{forge} is an embedded DSL in Scala for specifying other DSLs. Forge
is used by the Delite~\cite{delite} and LMS~\cite{lms, rompf13popl} compilation
frameworks. This approach requires DSL developers to learn a new specification
language before implementing DSLs.  
In contrast, \systemname developers write a DSL specification using \textit{plain}
Scala code. Then, domain-specific knowledge is encoded using simple \systemname
annotations. 

Yin-Yang~\cite{yinyang} uses Scala macros for automatically converting
shallow EDSLs to corresponding
deep EDSLs. 
Thus, it completely removes the need of providing the definition of a deep DSL
library from the DSL developer. However, contrary to our work, the compiler-compilation of Yin-Yang is specific to the LMS~\cite{lms} compilation framework. Also, Yin-Yang does not
generate any code related to optimizations of the DSL library. 
We have
identified the task of automatically generating the optimizations to be not only
a crucial requirement for DSL developers but also one that is significantly
more complicated than the one handled by Yin-Yang.

\todo{mention other work related to shallow vs. deep}
